What went wrong and when? Instance-wise Feature Importance for Time-series Models

Explanations of time series models are useful for high stakes applications like healthcare but have received little attention in machine learning literature. We propose FIT, a framework that evaluates the importance of observations for a multivariate time-series black-box model by quantifying the shift in the predictive distribution over time. FIT defines the importance of an observation based on its contribution to the distributional shift under a KL-divergence that contrasts the predictive distribution against a counterfactual where the rest of the features are unobserved. We also demonstrate the need to control for time-dependent distribution shifts. We compare with state-of-the-art baselines on simulated and real-world clinical data and demonstrate that our approach is superior in identifying important time points and observations throughout the time series.

==> experiment_old.tex <==
% \begin{table*}[!ht]
%     \centering
%     \begin{tabular}[t]{lccccc}
%          & \multicolumn{2}{c}{Spike Data} & \multicolumn{3}{c}{State Data} \\ 
%         \toprule
%         Method & AUROC (exp) & AUPRC (exp) & AUROC (exp) & AUPRC (exp) & Median Rank\\  \midrule
%         FIT (Ours) &  {\bf{ 0.9985 $\pm$ 0.0006}} & {\bf{0.8641 $\pm$ 0.0389}} &  {\bf{0.8196}}  &  {\bf{0.1535}} & 2\\
%         AFO &  0.9721 $\pm$ 0.0132 & 0.4406 $\pm$ 0.2819 &  0.7594 $\pm$ 0.0105  &  0.0357 $\pm$ 0.0025 \\
%         FO & 0.8913 $\pm$ 0.0013 &  0.3368 $\pm$ 0.162  &  0.7581 $\pm$ 0.012  & 0.0359 $\pm$ 0.0015 \\
%         SA & 0.6188 $\pm$ 0.0363  &  0.0372 $\pm$ 0.0036 &  0.716 $\pm$ 0.0044  &  0.0407 $\pm$ 0.0008 \\
%         LIME & 0.3403 $\pm$ 0.0072  &  0.001 $\pm$ 0.0 &  0.5659 $\pm$ 0.0141  &  0.0229 $\pm$ 0.004 \\ \bottomrule
% \end{tabular}
% \caption{Quantitative evaluation for simulated data using ground-truth feature importance. The proposed method detects important features with higher average precision compared to all baseline methods for both datasets, suggesting we capture the spike in the green feature (relevant feature and time) spike data and state changes along with important features in State Data more precisely than baselines.}
%     \label{tab:sim_results}
% \end{table*}{}


% \begin{table*}[!ht]
%     \centering
%     \begin{tabular}[t]{lcccc}
%          & \multicolumn{2}{c}{Spike Data} & \multicolumn{2}{c}{State Data} \\ 
%         \toprule
%         Method & AUROC (exp) & AUPRC (exp) & AUROC (exp) & AUPRC (exp)\\  \midrule
%         FIT (Ours) &  {\bf{ 0.9985 $\pm$ 0.0006}} & {\bf{0.8641 $\pm$ 0.0389}} &  {\bf{0.9269 $\pm$ 0.0094}}  &  {\bf{0.161 $\pm$ 0.025}} \\
%         AFO &  0.9721 $\pm$ 0.0132 & 0.4406 $\pm$ 0.2819 &  0.7594 $\pm$ 0.0105  &  0.0357 $\pm$ 0.0025 \\
%         FO & 0.8913 $\pm$ 0.0013 &  0.3368 $\pm$ 0.162  &  0.7581 $\pm$ 0.012  & 0.0359 $\pm$ 0.0015 \\
%         SA & 0.6188 $\pm$ 0.0363  &  0.0372 $\pm$ 0.0036 &  0.716 $\pm$ 0.0044  &  0.0407 $\pm$ 0.0008 \\
%         LIME & 0.3403 $\pm$ 0.0072  &  0.001 $\pm$ 0.0 &  0.5659 $\pm$ 0.0141  &  0.0229 $\pm$ 0.004 \\ \bottomrule
% \end{tabular}
% \caption{Quantitative evaluation for simulated data using ground-truth feature importance. The proposed method detects important features with higher average precision compared to all baseline methods for both datasets, suggesting we capture the spike in the green feature (relevant feature and time) spike data and state changes along with important features in State Data more precisely than baselines.}
%     \label{tab:sim_results}
% \end{table*}{}




\section{Evaluation}\label{sec:results}
We evaluate our feature importance assignment method (FIT) on $2$ simulated datasets, a real-world data set and a synthetic model, and a clinical dataset. For simulated data, ground-truth feature importance over time is available. Thus we directly evaluate our method by measuring the AUROC and AUPRC scores for identifying the important feature instances over time. We then apply our method to more complex clinical data to evaluate the performance on a real-world task. We compare with multiple groups of baseline methods, described below.

\begin{asparaenum}\label{list:baselines}
    \item {\bf{Perturbation-based methods:}}
    \begin{enumerate}[label=\alph*)]
        \item Feature Occlusion (FO): Introduced by ~\citet{suresh2017clinical}, this method is a perturbation-based method where importance is assigned based on the difference in model prediction when each feature $x_{i}$ is replaced with a random sample from the uniform distribution.
        \item Augmented feature occlusion (AFO): We augment the method introduced in~\citet{suresh2017clinical} by replacing observations with samples from the bootstrapped distribution $p(x_i)$ over each feature $i$. This avoids generating out-of-distribution samples.
    \end{enumerate}
    \item {\bf{Gradient-based methods:}}
    \begin{enumerate}[label=\alph*)]
        \item Deep Lift: a method designed specifically for neural networks, which decomposes the output on input features by backpropagating the contribution back to every feature of the input 
        \item Integrated gradient
    \end{enumerate}
    
    \item {\bf{Attention-based methods:}}
    \begin{enumerate}[label=\alph*)]
        \item RETAIN
    \end{enumerate}

    \item {\bf{Others:}}
    \begin{enumerate}[label=\alph*)]
        \item LIME~\citep{ribeiro2016should}: One of the most common explainabilty methods to assign local importance to features. Although LIME isn't designed to assign temporal importance, for this baseline, we use LIME at every time point for a fair comparison.
        \item Gradient-SHAP
    \end{enumerate}
\end{asparaenum}

\subsection{Simulated Datasets}\label{sec:simulation1}

Evaluating the quality of explanations is challenging due to the lack of a gold standard/ground truth for the explanations. Additionally, explanations are reflective of model behavior, therefore such evaluations are tightly linked to the reliability of the model itself. We therefore evaluate the functionality and performance of our baselines in a controlled simulated environment where the ground truth for feature importance is known. Experiment results on $2$ different simulations are presented below, followed by a comparison to attention mechanisms. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% SIMULATION I %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Simulated Data I: Spike Data}\label{res:sim1}

\begin{figure*}[!htbp]
    \centering
    \includegraphics[scale=0.05]{TS_explainability/Figures/simulated_results/legend_95_joint_RNN_generator.pdf}
    \includegraphics[scale=0.14]{TS_explainability/Figures/simulated_results/feature_95_joint_RNN_generator.pdf}
    \caption{Spike Data: Results from a sample from the dataset. Figure on the top shows the $3$ time series features and the dashed line indicates $y_t$, which switches from zero to one, only when the first spike apprears in the green feature ($0$) from a black-box prediction model. Each following row shows the importance assignment scores for our method (FIT) and the baselines. Each line in this subplot corresponds to the importance value for one of the features, indicated by the color, over time. FIT assigns high importance to the green feature at the exact time of first spike. FO fails to identify the green spike as the variance of its perturbations are too high to be sensitive to spikes. Detailed comparison is included Section~\ref{res:sim1} and Table~\ref{tab:sim_results}.}
    \label{fig:simulated_results1}
\end{figure*}
We simulate a time series data such that only one feature determines the outcome. Specifically, the outcome (label) changes to $1$ as soon as a spike is observed in the relevant feature. We keep the task fairly simple for two main reasons: 1) to ensure that the black-box classifier can indeed learn the right relation between the important feature and the outcome, which allows us to focus on evaluating the quality of the importance assignment without worrying about the quality of the classifier. 2) to have a gold standard for the explanations since the exact event predictive of the outcome is known.  We expect the explanations to assign importance to only the one relevant feature, at the exact time of spike, even in the presence of spikes in other non-relevant features. 
 
{\bf{Data generation:}} We generate $d=3$ (independent) sequences of standard non--linear auto-regressive moving average (NARMA) time series of the form:

\vspace{-1mm}
$x(t+1) = 0.5x(t) + 0.5x(t)\sum_{i=0}^{l-1} x(t-l) + 1.5u(t-(l-1))u(t) + 0.5$

for $t \in [80]$, where the order is $2$ and $u \sim \mathcal{N}(0, 0.01)$. We add linear trends to the features and introduce random spikes over time for every feature. We train an RNN-based black-box predictor with AUC$ =0.99$, and choose feature $0$ (green on the plots) to be the important feature that determines the output $y_t$. The full procedure is described in Appendix~\ref{sec:appendix_sim2}.
\begin{figure*}[!htbp]
    \centering
    \includegraphics[scale=0.05]{TS_explainability/Figures/simulated_results/legend_23.pdf}
    \centering
    \includegraphics[scale=0.14]{TS_explainability/Figures/simulated_results/feature_23_joint_RNN_generator.pdf}
    \caption{State Data: The top plot shows the time series signals and the output risk of the black-box model. Shaded regions indicate different hidden sates of the Markov model. The 4 lower plots are the importance assignments for FIT and other baselines. FIT assigns high importance at the exact critical time points of state change. AFO an FO are only able to find the most important feature in every state, but not the important time. And sensitivity analysis only detects the importance of later observations.}
    \label{fig:simfig2}
\end{figure*}
{\bf{Experiment results:}} Figure~\ref{fig:simulated_results1} demonstrates explanations from each of the compared approaches for an illustrative samples from the testset. Note that all baseline methods provide an importance for every sample at each time point. The true explanation is to highlight the green feature at the time of the first spike. Using this ground truth, we evaluate the AUROC and AUPRC of the generated explanations. Table~\ref{tab:sim_results} summarizes these results. From Figure~\ref{fig:simulated_results1}, we see that FIT identifies the right explanation by assigning importance to the green feature at the exact time of spike. FO fails to recover the important observation, and assigns random importance values to all features. This is due to the variance of perturbations drawn from the uniform distribution. AFO improves over this, by sampling from the marginal distribution which is more representative of the signals. This explains why it can identify the spike, and assigns more precise importance to features, compared to FO. Even if AFO ignores temporal dynamics, for this task, the conditional distribution modeled by FIT is reasonably approximated by the marginal. However, the magnitude of feature importance is not meaningful, resulting in the lower average precision of AFO in Table~\ref{tab:sim_results}. Note that importance value for all features become zero after the spike, since nothing can change the output after that. Sensitivity analysis is gradient-based and can only capture changes to the prediction reliably for infinitesimally small perturbations, and not temporal dynamics. This baseline is thus able to locate the important time of spike in the green feature, however, the actual magnitude of gradient based importance values doesn't distinguish the relative importance of the different features over time. More examples are provided in the Appendix~\ref{app:sim1}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% SIMULATION II %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Simulated Data II: State Data}\label{sec:simulation2}
The first simulation ensures correct functionality of the method but does not necessarily evaluate it under complex state dynamics that is common in real-word time-series data. In this simulation, we create a dataset with a more complex temporal dynamics. 

{\bf{Data generation:}} The dataset consists of multivariate time series signals with $3$ features. We use a non--stationary Hidden Markov Model with $2$ latent states, and a linear transition matrix to generate observations over time. Specifically, at each time step $t$, observations are sampled from the multivariate normal distribution determined by the latent state of the HMM at that time. The non-stationarity models the state transition probabilities as a function of time. The outcome $y$ is a Bernoulli random variable, which, in state $1$, is only determined by feature $1$, and in state $2$, by feature $2$. The ground truth explanation for output at time $T$ is the observation $x_{i,t}$ where $i$ is the important feature for the current state and $t$ indicates when feature $i$ became important (state change). A full explanation for outcome at $t=T$ should include the most important feature variable as well as the time point of importance.

{\bf{Experiment results:}}

% Figure~\ref{fig:simfig2} shows the assigned importance for different features of the time series sample. The top plot is the time series data and shaded regions indicate the hidden state of the Markov model. The following rows show feature importance evaluation results for each baseline. AFO and FO capture the important feature in every state. However neither method characterizes temporal dynamics of the signal. The top importance values from each method therefore do not correspond to the state changes, i.e. important time points. The Sensitivity Analysis baseline is biased toward later observations, and therefore misses earlier state changes. This is because RNN-based black-box predictors are less sensitive to long source dependencies due to vanishing saliency~\cite{ismail2019input}. Only FIT assigns high relative importance to features at times which corresponding to state changes. Table~\ref{tab:sim_results} compares performance across our baselines, measured as AUROC and AUPRC scores indicating the number of correct explanations assigned by each method. FIT provides a considerable improvement over all baselines in this task. Note that the AUPRC values are small for all methods, which is due to vast imbalance in false positive importances for the baseline methods.

\begin{table*}[!ht]
    \centering
    \begin{tabular}[t]{lcccc}
        \toprule
        Method & AUROC (explanation) & AUPRC (explanation) & AUROC drop (black-box) & Accuracy drop (black-box)\\  \midrule
        FIT (Ours) &  {\bf{ 0.9985 $\pm$ 0.0006}}& \\
        \midrule
        AFO  &  & \\
        FO  &  & \\
        \midrule
        Deep Lift  &  & \\
        Integrated Gradient  &  & \\
        \midrule
        RETAIN  &  & \\
        \midrule
        LIME  &  & \\
        SHAP Gradient  &  & \\
        \bottomrule
\end{tabular}
\caption{AUC drop for baselines}
    \label{tab:sim_results}
\end{table*}{}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% Explaining Attention %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[]
    \centering
    \begin{tabular}{lcc} \toprule
         \multicolumn{3}{c}{Spike Data} \\ 
        \toprule
        Method & AUROC (exp) & AUPRC (exp) \\  \midrule
        FIT (Ours) &  0.986 $\pm$ 0.0005  &  {\bf{0.566 $\pm$ 0.0025}} \\ 
        Attention &  {\bf{0.9908 $\pm$ 0.0001}}  &  0.2651 $\pm$ 0.0002 \\ 
        AFO &  0.9162 $\pm$ 0.0096  &  0.0411 $\pm$ 0.0018 \\ 
        FO &  0.9099 $\pm$ 0.0033  &  0.1447 $\pm$ 0.0304 \\ 
        SA &  0.7735 $\pm$ 0.0348  &  0.0613 $\pm$ 0.0274 \\ 
        LIME &  0.3756 $\pm$ 0.0114  &  0.0014 $\pm$ 0.0 \\ \bottomrule
\end{tabular}
    \caption{Spike Data: Compared to attention scores, FIT provides more precise time importance, along with feature importance.}
    \label{tab:sim1_attention}
\end{table}{}


\vspace{-2mm}


\begin{table}[]
    \centering
    \begin{tabular}{lcc}
          \multicolumn{3}{c}{State Data} \\ 
        \toprule
        Method & AUROC (exp) & AUPRC (exp) \\  \midrule
        FIT (Ours) &  {\bf{0.9482 $\pm$ 0.0047}}  &   {\bf{0.5407 $\pm$ 0.0112}}\\
        Attention & 0.6522 $\pm$ 0.0358  &  0.1827 $\pm$ 0.0156 \\ 
        AFO &  0.7786 $\pm$ 0.0287  &  0.1896 $\pm$ 0.0096\\ 
        FO &  0.7608 $\pm$ 0.0311  &  0.1658 $\pm$ 0.0146\\ 
        SA &  0.8061 $\pm$ 0.0169  &  0.2109 $\pm$ 0.0188\\ 
        LIME  &  0.4762 $\pm$ 0.0006  &  0.0504 $\pm$ 0.0009 \\ \bottomrule
\end{tabular}
    \caption{State Data: Comparison of attention scores, FIT provides the exact time instances of state changes whereas Attention focuses on all observations in a given state that predict the outcome.}
    \label{tab:sim2_attention}
\end{table}{}


\subsubsection{Explaining Attention Model}\label{sec:attention_baseline}
Attention Models~\cite{bahdanau2014neural,vaswani2017attention}, that are primarily used for seq2seq tasks in NLP, have also shown success in prediction tasks using time series~\cite{song2018attend,choi2016retain}. In addition to improving performance, the attention weights can also be used to determine the importance of observations over time. However, in time series, they do not distinguish the relative importance of features at each time point. In this section, we compare generated explanations of different methods to the importance values assigned by attention weights over time. For this purpose, we train an Attention model as the black-box predictor for the same simulated data. We explain this black-box predictor and compare the performance for time importance assignment across all methods, including the attention weights of the black-box model. The results on Simulated Data are summarized in Table~\ref{tab:sim1_attention}and~\ref{tab:sim2_attention}. The results show that even in explaining an attention model, our proposed method assigns time importance with much higher average precision than the attention weights. This is because the attention model assigns high weights to all observations that lead to the outcome, and fails to identify the most informative observation over time.
\begin{figure}[t]
\centering
    \includegraphics[scale=0.23]{TS_explainability/Figures/mimic_results/heatmap_619_FFC.pdf}
    \caption{Heatmap explaining the mortality prediction model using FIT. Results show the importance assignment for each feature at every hour for a sample patient shown in Figure~\ref{fig:mimic}.}
    \label{fig:mimic_heatmap}
\end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% MIMIC Dataset %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[h]
\centering
        \includegraphics[scale=0.32]{TS_explainability/Figures/mimic_results/legend_619_joint_RNN_generator.pdf}
        \includegraphics[scale=0.14]{TS_explainability/Figures/mimic_results/feature_619_joint_RNN_generator.pdf}
    \caption{MIMIC III: The top row shows the output risk of the prediction model (black dashed line), and normalized time series signals. The four bottom rows correspond to importance scores generated by each of the methods and the error bars indicate the standard deviation of the importance value.FIT, AFO and FO find similar features important. Sensitivity analysis identifies the critical point but is unable to attribute the importance to appropriate features reliably.}
    \label{fig:mimic}
\end{figure*}

{\color{red} TODO: \subsubsection{Quality of the Generator/Hypothesis testing}}

{\color{red}\subsection{ TODO: Semi-synthetic Time-Series Classification}}

\subsection{MIMIC Mortality Prediction Model}\label{sec:mimic_mortality}

Explaining models based on feature and time importance is critical for clinical settings. Therefore, having verified performance quantitatively on simulated data, we test our methods on a more complex mortality prediction task for the Intensive Care Unit (ICU). The black-box model is an RNN-based mortality prediction model, trained on time series data from the MIMIC-III dataset. The data consists of de-identified EHRs for $\sim40,000$ ICU patients at the Beth Israel Deaconess Medical Center, Boston, MA and includes time series measurements such as vitals and lab results over patients' ICU stay~\citep{johnson2016mimic}. The RNN-based black-box model uses static patient information (age, gender, ethnicity), $8$ vital measurements and $20$ lab results to predict mortality in the next 48 hour. Further details on the model and data can be found in Appendix~\ref{app:mimic}.

Following the procedure in Algorithm~\ref{alg:algo1}, we train a conditional generator for the time series features (vitals and lab measures) to assign importance over time using FIT. Figure~\ref{fig:mimic_heatmap} shows a sample heatmap of the importance of each clinical measurement, at every hour during a patient's ICU stay (assigned by our method). Similar heatmap results for other baselines are also provided in Appendix~\ref{app:mimic}. 
To compare results across different methods, we also look into the importance assignment of our baselines in Figure \ref{fig:mimic}. The top plot shows the trajectory of multiple signals for this specific individual, and the dashed black line indicates the model prediction. The plots below visualize importance scores over time for the top most important signals.

As shown in Figure \ref{fig:mimic},  AFO, FO and FIT pick almost the same signals as important features for this individual patient and the importance peaks around similar time. While sensitivity analysis identifies the critical time point, it fails to infer the correct relative importance for the features. Due to lack of ground truth for explanations, we use global importance as a proxy for evaluation. In future work, this evaluation can be done with the help of domain experts, i.e. ICU clinicians.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% Global Importance %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[!ht]
\centering
\begin{tabular}{lcc}
\toprule
{\bf{Method}} & \begin{tabular}[c]{@{}l@{}}AUROC -model\\ w/o top $10$ \\ (lower is better)\end{tabular} & \begin{tabular}[c]{@{}l@{}}AUROC -model\\ w/ top $3$ only\\ (higher is better)\end{tabular} \\ \midrule
FIT & {\bf{0.7787 $\pm$ 0.0008}} & 0.7206 $\pm$ 0.0012 \\ 
AFO & 0.7796 $\pm$ 0.0004 & {\bf{0.7217 $\pm$ 0.0009}}\\
FO & 0.7855 $\pm$ 0.0012 & 0.7203 $\pm$  0.0007\\ 
SA & 0.7816 $\pm$ 0.0028 & 0.6939 $\pm$ 0.0009\\ 
LIME & 0.7808 $\pm$ 0.0024 & 0.6797 $\pm$ 0.0003 \\ \bottomrule
\end{tabular}
    \caption{\small{Real Data - Global Importance. Prediction model deteriorates the most when top $10$ features according to FIT are removed suggesting it reliably captures global relevance and provides competitive performance, just after AFO when trained only on top $3$ features according to FIT.}}
    \label{tab:mimic_global_results}
    \vspace{-2.5mm}
\end{table}

\subsubsection{Evaluation Using Global Importance}
Another way to quantitatively evaluate the proposed method on real data, is to assess how well the method performs at selecting \emph{globally} important features. We evaluate global importance by studying \begin{inparaitem}\item[i)] how much the prediction model performance deteriorate if the top $10$ most relevant features according to each method are removed (lower is better) and \item[ii)] how well the prediction model performs if trained using only the top $3$ relevant features determined by the method (higher is better)\end{inparaitem}. The results in Table~\ref{tab:mimic_global_results} demonstrate that the proposed method is competitive at assigning population level importance.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% Sanity Check %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.36]{TS_explainability/Figures/simulated_results/sanity_checks.pdf}
    \caption{Parameter randomization sanity check. The x-axis indicates the portion of the network parameters that are randomized, and the y-axis shows the Spearman rank correlation of the explanations of the randomized model with the original explanation.}
    \label{fig:sanity_check}
\end{figure}{}

{\color{red}\subsection{TODO: Calibration of importance scores compared to baselines}}

\subsection{Sanity Check Test for Explanations}
We additionally evaluate the quality of the proposed FIT method using the parameter randomization test proposed as `Sanity Checks' in \cite{adebayo2018sanity}. We use cascading randomization by gradually randomizing model weights and evaluating the rank correlation of explanations generated on the randomized model to the explanation of the original model. A method is reliable if its explanations of the randomized model and original model are uncorrelated, with increased randomization further reducing the correlation between explanations. Figure \ref{fig:sanity_check} demonstrates that our method passes this check as the explanations from the randomized models have little correlation with the original explanations.
\vspace{-8mm}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

